Statistics of modal condensation in nonlinear multimode fibers

Optical pulses propagating in multimode optical fibers are affected by linear disorder and nonlinearity, and experience chaotic exchange of power among modes. On the other hand, complex systems can attain steady states characterized by energy condensation into single as well multiple sub-systems. In this work, we study beam propagation in multimode optical fibers in the presence of linear random mode coupling and Kerr nonlinearity; both effects lead to a mode power redistribution at the fiber output. We use a new 3D mode decomposition method to obtain, with unprecedented accuracy, measurements of the modal distribution from long spans of graded-index fiber; we perform numerical simulations using a new model for the linear disorder; we introduce a weighted Bose-Einstein law and show that it is suitable for describing steady-state modal power distributions both in the linear and nonlinear regimes. We show that, at power levels intermediate between the linear and the soliton regimes, energy condensation is attained locally by the second, third and fourth modal groups, before global condensation to the fundamental mode is reached in the soliton regime. Our results extend the thermodynamic approach to multimode fibers to unexplored optical states, which acquire the characteristics of optical glass.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} D. Gloge, Bending Loss in Multimode Fibers with Graded and Ungraded Core Index, Appl. Opt., 11(11) (1972) 2506-2513.

\bibitem{bib2} D. Flamm, D. Naidoo, C. Schulze, A. Forbes, M. Duparr, Mode analysis with a spatial light modulator as a correlation filter, Opt. Lett. 37(13) (2012) 2478--2480.

\bibitem{bib3} M. ZItelli, V. Couderc, M. Ferraro, F. Mangini, P. Parra-Rivas, Y. Sun, S. Wabnitz, Spatiotemporal mode decomposition of ultrashort pulses in linear and nonlinear graded-index multimode fibers, Phot. Res., 11(3) (2023) DOI 10.1364/PR.484271

\bibitem{bib4} D. Marcuse, Losses and impulse response of a parabolic index fiber with random bends, Bell Sys. Tech. Journ., 52(8) (1973) 1423-1437.

\bibitem{bib5}

\bibitem{bib6} 

\bibitem{bib7} 


%\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

%\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

%\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

%\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

%\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

%\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

%\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.

\end{thebibliography}


